Can We Generate Shellcodes via Natural Language? An Empirical Study

Writing software exploits is an important practice for offensive security analysts to investigate and prevent attacks. In particular, shellcodes are especially time-consuming and a technical challenge, as they are written in assembly language. In this work, we address the task of automatically generating shellcodes, starting purely from descriptions in natural language, by proposing an approach based on Neural Machine Translation (NMT). We then present an empirical study using a novel dataset (Shellcode_IA32), which consists of 3,200 assembly code snippets of real Linux/x86 shellcodes from public databases, annotated using natural language. Moreover, we propose novel metrics to evaluate the accuracy of NMT at generating shellcodes. The empirical analysis shows that NMT can generate assembly code snippets from the natural language with high accuracy and that in many cases can generate entire shellcodes with no errors.

==> tex/approach_old.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1\linewidth]{img/approach.pdf}
\caption{Architecture diagram of the approach demonstrating a six-step process: 1) Pre-Processing of the samples in the training data, 2) Training of the neural machine translation system with the processed training data, 3) User stating the operation in the English language (i.e., the \textit{intent}), 4) Pre-processing of the intent, 5) NMT models generating the \textit{code snippet} from the processed intent, and lastly, 6) Output after post-processing applied to the generated code snippet.}
  \label{fig:approach}
\end{figure*}



The approach leverages neural machine translation (NMT) to automatically generate exploits. A neural machine translation system is a neural network that maximizes the conditional probability $p(a|e)$ of translating a source sentence $e = <e_1,...,e_{T_e}>$, with length $|e| = T_e$, into a target sentence $a = <a_1,...,a_{T_a}>$, with length $|a|= T_a$.
%The goal of an NMT system is to take in input a sequence $e = <e_1,...,e_{T_e}>$ of tokens in a source language, with length $|T_e|$, and to find a token sequence $\hat{a} = a_1,...,a_{T_a}$ in a target language, with length $|T_a|$, so that: 
%\begin{equation}
%\label{eq:problem}
%\hat a =\underset{a}{\text{argmax}}\, log\, p(a\, |\, e)
%\end{equation}
%Following prior work (e.g.~\cite{luong2015effective}), we build a neural network that directly models the conditional probability $p(a|e)$ of translating an input sequence of tokens (an \emph{intent}, in natural language) to a target sequence of Python or assembly language tokens (a \emph{code snippet}). 
Following prior work (e.g.,~\cite{luong2015effective}), we build a neural network that directly models the conditional probability $p(a|e)$ of translating an \emph{intent}, in natural language into a \emph{code snippet} in assembly language.
As a simple example, consider the sequence of English tokens {\fontfamily{qcr} \small\selectfont [`add', `the', `value', `4', `to', `the', `eax', `register']} as $e$, and the sequence of assembly tokens {\fontfamily{qcr} \small \selectfont [`add', `eax', `,', `4']} as $a$, with $|e|=8$ and $|a|=4$. 
The general architecture of an NMT system consists of an encoder, which computes a representation $s$ for each source token, and a decoder, which generates tokens in the target language. 
%The NMT system generates one target token at a time, by decomposing the probability as in:
%\begin{equation}
%\label{eq:decoding}
%\log p(a|e) =\sum_{t=1}^{T_a} \log p(a_t|a_{<t},s)
%\end{equation}

%Given an English intent $e$, our problem is to find a token sequence $\hat{a}$ so that: 
%\begin{equation}
%\label{eq:problem}
%\hat a =\underset{a}{\text{argmax}}\, log\, p(a\, |\, e)
%\end{equation}
%Here $log\, p(a\, |\, e)$ is estimated by the model using Equation~\ref{eq:decoding} (see \S~\ref{subsec:model}). 
%We define $a = a_1,...,a_{T_a}$  as a Python code or assembly code token sequence with length $|T_a|$. We define $e = e_1,...,e_{T_e}$ as a natural language token sequence with length $|T_e|$.

To support automatic code generation, neural machine translation is usually accompanied by data processing steps \cite{park2020decoding,8713737,oudah2019impact}. These phases strongly depend on the specific source and target languages to translate (in our case, exploit code from the English language). The approach applies steps of processing both before the NMT task (\textit{pre-processing}), to train the NMT model and prepare the input data, and after the NMT task (\textit{post-processing}), to improve the quality and the readability of the code in output. 
Figure~\ref{fig:approach} shows the architecture of our approach, along with an example of inputs and outputs at each step, further discussed in the following.




\subsection{Pre-Processing}
\label{subsec:preprocessing}

%Pre-processing and post-processing are significant aspects of natural language processing application software \cite{park2020decoding}. 
%Pre-processing in neural machine translation includes subword tokenization to alleviate the problem of unknown words, parallel corpus filtering that only filters data suitable for training, and data augmentation to ensure that the corpus contains sufficient content.


Pre-processing starts with \textit{stopwords filtering}, i.e., by removing a set of custom compiled words (e.g., \textit{the, each, onto}), in order to include only relevant data for machine translation. %...for training the NMT models and to aid the model in improving the accuracy for the output prediction. 
%During the experimentation phase, snippets, and intents went through several steps that were omitted later on as they did not affect performance. The steps include stemming, punctuation removal, tokenization \cite{kudo2018sentencepiece} using word and sub-words algorithms (the Unigram Language Model \cite{DBLP:journals/corr/abs-1804-10959}). \pietro{Is it necessary? Need to explain what they are.} 
This phase splits the input sequence of natural language tokens $e_1,...,e_{T_e}$ and code into $a_1,...,a_{T_a}$ in a process called \textit{tokenization}. 
%For the sequence-to-sequence model (\S~\ref{subsec:model}), we tokenize using \textit{Byte Pair Encoding} (BPE) \cite{sennrich-etal-2016-neural}. 
%For CodeBERT (\S~\ref{subsec:model}), we use a variant of the BPE, the RoBERTa tokenizer ~\cite{liu2019roberta}. 
The tokenizer converts the input strings into their byte representations, and learns to break down a word into subword tokens (e.g., lower becomes \texttt{[low,er]}. 
We tokenize intents using the \textit{nltk word tokenizer} \cite{loper2002nltk} and snippets using the Python \textit{tokenize} package \cite{tokenize}. We then use regular expressions to identify hexadecimal values (e.g., \texttt{0xbb}), strings that fall between quotation marks, squared brackets, variable name notations (e.g., \texttt{variableName}, \texttt{variable\_name}), follow underscore notation (e.g., \texttt{next\_cycle}), function names, mathematical expressions, and byte arrays (e.g., \texttt{\textbackslash xe3 \textbackslash xa1}). We also use WordNet \cite{miller1995wordnet} to recognize alphabet strings that do not belong to the English language. 


Consider the natural language intent shown in Figure~\ref{fig:approach} (step \circled{3}), which contains the phrase \emph{jump to \texttt{next\_cycle}}. 
One task for code generation systems is to prevent non-English tokens (e.g., \texttt{next\_cycle}) from getting transformed during the learning process. This process is known as \textbf{\textit{Standardization}}. Extant code generation systems address this problem with \emph{copying} mechanisms in neural network architectures \cite{gu2016incorporating}, which are inspired by human memorization. %However, since resources like abstract syntax parser for assembly language do not yet exist \cite{jia2016data}, ...
To perform standardization, the approach provides a novel \textbf{\textit{Intent Parser}} tailored for working with exploit software. 
The goal of the Intent Parser is to take input in natural language (i.e. intents) and to provide as output a dictionary of standardizable tokens, such as specific values, label names, and parameters.% (e.g., it recognizes \texttt{next\_cycle} as a standardizable token, \texttt{var2}). 

All tokens selected by the Intent Parser are passed to the \textbf{\textit{Standardizer}}. The standardization process simply replaces the selected token in both the intent and snippet with \texttt{var\#}, with \texttt{\#} denoting a number from $0$ to $|l|$, and $|l|$ is the number of tokens to standardize.  
In the step~\circled{4} in \figurename~\ref{fig:approach}, the intent parser identifies \texttt{dl}, \texttt{0xbb}, and \texttt{next\_cycle} as standardizable tokens and standardizes them to \texttt{var0}, \texttt{var1}, and \texttt{var2} respectively (based on order of appearance in the intent). 
To prevent the standardization of unimportant tokens, we compile a dictionary of $45$ assembly keywords (e.g., \texttt{register}, \texttt{address}, \texttt{byte}) as non-standardizable tokens. 
After the standardization process, both the original token and its standardized counterpart (\texttt{var\#}) are stored in a dictionary %called \textbf{Slotmap} 
to be used during post-processing.

%Lastly, we create \textit{\textbf{Embeddings}}, which are numerical representations for each token in both the intent and snippet sequences.
%These representations are created by converting tokens into numerical ids.
Lastly, we create \textit{\textbf{Embeddings}}, i.e., a mapping of each token (in both the intent and code snippet sequences) into a numerical id representation in order to capture their semantic and syntactic information, where the semantic information correlates with the meaning of the tokens, while the syntactic one refers to their structural roles \cite{li2018word}.


\subsection{NMT Models}
\label{subsec:model}

To perform neural machine translation (step \circled{5}), we consider two standard architectures: Seq2Seq, and CodeBERT.


\textbf{Seq2Seq.} Seq2Seq is a common model used in a variety of neural machine translation tasks. Similar to the encoder-decoder architecture with attention mechanism \cite{bahdanau2014neural}, we use a bi-directional LSTM as the encoder, to transform an embedded intent sequence $e = |e_1,...,e_{T_e}|$ into a vector $c$ of hidden states with equal length. 
Within the bidirectional LSTM encoder, each hidden state $h_t$ corresponds to an embedded token $e_t$. The encoder LSTM is bidirectional, which means it reads the source sequence $e$ ordered from left to right (from $e_1$ to $e_{T_e}$) and from right to left (from  $e_{T_e}$ to $e_1$). To combine both directions, each hidden state for the bidirectional LSTM encoder is computed by concatenating the hidden states of the forward and backward orders at token $t$ as follows:
\begin{equation}
\label{eq:encoding}
\begin{matrix}
\textbf{h}_t = [f(e_t,\textbf{h}_{t-1}) ; f(e_t,\textbf{h}_{t+1})] ;  
% \\
% \textbf{c} = \phi(\{\textbf{h}_1, ..., \textbf{h}_{T_S}\}) 
\end{matrix}
\end{equation}
where $h_t$ denotes a hidden state at time step $t$, $e_t$ denotes an embedded intent token $t$, and $f$ denotes an LSTM non-linear function. 
% To enhance the model's capabilities on longer sequences, 
Next, the model generates a context vector $c_t$ for each of the embedded inputs.  We use the Bahdanau-style attention mechanism \cite{bahdanau2014neural}, %in which it considers a dynamic context $\textbf{c}_t$ in the decoding process.  This attender attends to the entire input space (i.e. 
which uses soft attention by representing $\textbf{c}_t$ as the weighted sum of the encoder hidden states, as $\mathbf{c}_t = \sum_{i=1}^{{T_e}} \alpha_{t,i}\: \textbf{h}_i$, where the scores $\alpha_{t,i}$ are parametrized by a feed-forward multi-layer perceptron neural network. Since the encoder uses a bidirectional LSTM, each hidden state $\textbf{h}_i$ is aware of the context on both ends.

%\begin{equation}
%\label{eq:attention}
%\begin{matrix}
%\mathbf{c}_t = \sum_{i=1}^{{T_e}} \alpha_{t,i}\: %\textbf{h}_i \\ \\
%%\alpha_{t,i} = \frac{\exp(score(\textbf{s}_{t-1}, \textbf{h}_i))}{\sum_{i'=1}^n \exp(score(\textbf{s}_{t-1}, \textbf{h}_{i'}))}
%\alpha_{t,i} = softmax(score(\textbf{s}_{t-1},\textbf{h}_i)) \\ \\
%score(\textbf{s}_{t},\textbf{h}_i) = v_{z}^{\top} tanh(\textbf{W}_z[\textbf{s}_t; \textbf{h}_i])
%\end{matrix}
%\end{equation}

%where $\alpha_{t,i}$ represents how well a target token $a_t$ and source token $e_i$ align, $T_e$ represents the last hidden state in the LSTM encoder network,  $s_t$ is the decoder LSTM state at time step $t$, and lastly, $v_z$ and $W_z$ are weight matrices to be learned by the alignment model. The score $\alpha_{t,i}$ is parametrized by a feed-forward multi-layer perceptron neural network. Since the encoder uses a bidirectional LSTM each hidden state $\textbf{h}_i$ is aware of the context on both ends.  


%%LSTM (recurrent neural network (RNN) architecture)
The decoder generates one target token at a time by decomposing the conditional probability $p(a|e)$ into $\prod_{t=1}^{T_a} p(a_t|a_{<t},s)$, where $a_t$ is an individual output token. 
The target token are generated by combining the LSTM decoder state $s_{t-1}$, the previously-generated token $a_{t-1}$, and the context vector $c_t$ as follows:
\begin{equation}
\label{eq:seq2seq}
\begin{matrix}
\textbf{s}_t = f(a_{t-1},\textbf{s}_{t-1}, \textbf{c}) \\ \\
\: \: \: \: \: \:  p(a_t|a_{<t},e) = g( a_{t-1},\textbf{s}_t,\textbf{c})
\end{matrix}
\end{equation}

\noindent
where $g$ is a non-linear function, and  $a_{<t}$ denotes previous predicted tokens $\{a_1,...,a_{t-1}\}$.





%\ea{Insert Transformer architecture diagram? Note -- I do not mention all the hyperparameter dimension sizes for the formulas unless they are described in CodeBERT. I also don't mention normalization throughout the process. I hope this initial draft makes sense.}







%Such large models undergo a process called \emph{pre-training}, in which the models utilize massive amounts of unlabeled text and unsupervised learning to learn effective contextual representations of text. 

%Large pre-trained models such as ELMo~\cite{peters2018deep}, RoBERTa~\cite{liu2019roberta}, BERT~\cite{devlin2018bert}, and more recently GPT-3 ~\cite{brown2020language} have pushed the boundaries for state-of-the-art in natural language processing. 


%CodeBERT has been shown to achieve state-of-the-art on the task of generating code documentation given snippets as well as retrieving code snippets given a natural language search query across six different programming languages~\cite{husain_codesearchnet_2019}.

\textbf{CodeBERT.} CodeBERT~\cite{feng_codebert_2020} is a large multi-layer bidirectional Transformer architecture~\cite{vaswani2017attention}. Like Seq2Seq, the Transformer architecture is made up of encoders and decoders. CodeBERT has 12 stacked encoders and 12 stacked decoders. Compared to Seq2Seq, the Transformer architecture introduces mechanisms to address key issues in machine translation: (i) the translation of a word depends on its position within the sentence; (ii) in the target language, the order of the words (e.g., adjectives before a noun) can be different from the order of words in the source language (e.g., adjectives after a noun); (iii) several words in the same sentence can be correlated (e.g., pronouns). These problems are especially important when dealing with long sentences.

The Transformer architecture first refines the input embedding of each token, by combining it with a \emph{positional encoding} vector. The architecture has a different positional encoding vector for each position of the sentence, in order to enrich the input embedding with positional information. Then, the transformed input embeddings sequentially go through the stacked encoder layers, which all apply a \emph{self-attention} process. The self-attention further refines an input embedding, by combining it with the other input embeddings for the sentence in a weighted way, in order to account for correlations among the words (e.g., to get information for a pronoun from the noun it refers to, the input embedding of the noun is given a large weight). The weights are given by:

\begin{equation}
\label{eq:transformers_attention}
Attention (Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_k}})V
\end{equation}

\noindent
where the vectors $Q$ (query), $K$ (key), and $V$ (value) are learned during training. To further improve this mechanism, the Transformer architecture uses \emph{multi-headed attention}, where input embeddings are first multiplied with three learned weight matrices $W_{i}^Q$, $W_{i}^K$, and $W_{i}^V$ (where $i$ is a ``head''), then combined with vectors $Q$, $K$, and $V$. Finally, the results from all heads are concatenated and multiplied with an additional weights matrix $W^O$. Multi-headed attention enables the neural network to correlate different parts of the sequence in different ways (e.g., short-term vs long-term correlations). 

\begin{equation}
\label{eq:transformers_multiattention}
MultiHead (Q,K,V) = Concat(head_1,...,head_h)W^O
\end{equation}


% Each token in a sequence has an embedding vector. An embedding is a numerical form of a word that preserves its meaning by using dimensionality reduction and maintaining context. The paper uses 512 dimensions for the embedding size ($d_{model} = 512$). Each attention head takes in 3 input vectors for each input token: the query vector $Q$, the key vector $K$, and the value vector $V$. Each of these vectors has a dimension of 64. These vectors are computed by multiplying the embedded input token with 3 different weight matrices: $W^Q$, $W^K$, and $W^V$ respectively. The output of the attention head is computed as a weighted sum of the values vector. $d_k$ is the dimension of the key vectors which is 64.

%Following computing multi-headed attention, the result is fed into a feed-forward network and is fed into the next encoder and the process is repeated. Once the process in the final encoder (12th) layer is completed, the output of the 12th encoder layer is fed into each of the 6 decoders. The decoder also receives embedded target utterances after going through positional encoding. Similar to the encoder architecture each of the 6 decoders has a multi-layer perceptron network, multi-headed attention, and masked self-attention. The masked self-attention similar to the multi-headed attention attends to the output sequence with a tweak preventing the model from attending to subsequent output tokens. In other words, it only attends to the current output token and the past tokens.



Different from Seq2Seq, CodeBERT also comes with a \emph{pre-trained} neural network model, learned from large amounts of code snippets and their descriptions in the English language, and covering six different programming languages, including Python, Java, Javascript, Go, PHP, and Ruby. The goal of pre-training is to bootstrap the training process, by establishing an initial version of the neural network, to be further trained for the specific task of interest \cite{peters2018deep,liu2019roberta,devlin2018bert,brown2020language}. This approach is called \emph{transfer learning}. In our case, we fine-tune the CodeBERT model to translate English assembly using our exploit dataset (see \S{}~\ref{sec:dataset}).

%Thus, the model is pre-trained in a particular setting (e.g., general-purpose Python) and is fine-tuned on another similar task (e.g., Python for exploit code).

%The pre-training objectives for CodeBERT are then combined into one loss function as follows:
%\begin{equation}
%\underset{\theta}{min} \;\; L_{MLM} (\theta) + L_{RTD} (\theta) 
%\end{equation}

CodeBERT undergoes unsupervised pre-training using two optimization objectives: a \textit{masked language modeling} (MLM) objective~\cite{devlin2018bert} and a \textit{replaced token detection} (RTD) objective ~\cite{clark2020electra}. These two objectives are combined into one loss function $\underset{\theta}{min} \;\; L_{MLM} (\theta) + L_{RTD} (\theta)$.


The MLM objective selects random positions within the intent word sequence $e$ and code snippet sequence $c$, and replaces them with a special mask token $[MASK]$. %until approximately $15\%$ of the tokens within both $i$ and $s$ is masked out. 
The objective of this pre-training is to predict the original tokens that were replaced with $[MASK]$:

\begin{equation}
\label{eq:transformers_mlm}
L_{MLM} (\theta) = \sum_{i \in m^e \bigcup m^c} - \log p^{D_1} (x_i | e^{masked} , c^{masked})
\end{equation}

\noindent
where $p^{D_1}$ is the model that predicts the masked tokens, $m^e$ and $m^c$ are the randomly selected positions, $x = \{e,c\}$ is the original intent-snippet pair, and $e^{masked}$ and $c^{masked}$ are the masked intent and snippet.
%The second pretraining objective for CodeBERT is to replace token detection (RTD). Just like in the masked language modeling objective a set of tokens will be masked. 

In the RTD objective, both the intent and snippet are corrupted by replacing the original token with incorrect ones, and the trained model is used as a \emph{discriminator} (denoted as $p^{D_2}$) to detect whether a token is original or replaced. To this purpose, CodeBERT uses two \emph{generator} models (similarly to Generative Adversarial Networks), one for intents $p^{G_e}$ and one for snippets $p^{G_c}$. The generator models are trained to generate plausible token fits for the masked tokens $e^{masked}$ and $c^{masked}$. % in an intent-snippet pair $x$ respectively. $x_{corrupt}$ will be the sample upon replacing the masked tokens  $e^{masked}$ and $c^{masked}$ with generated tokens using the models  $p^{G_e}$ and  $p^{G_c}$ respectively.
The RTD objective is defined as follows:

\begin{equation}
\label{eq:transformers_RTD}
\begin{matrix}
L_{RTD} (\theta) = \mathlarger{\sum}_{i = 1} ^{|e| + |c|} \Big(\sigma(i) \log p^{D_2}  (x_{corrupt}, i) + \big( 1 - \sigma(i)\big)\\ \big(1 - \log p^{D_2} (x^{corrupt} , i ) \big) \Big)\\ \\
\sigma (i) = \Big\{\begin{matrix} 1, \; \;  \mathrm{if} \; x_i^{corrupt} = x_i\\0, \; \; \mathrm{otherwise.}
\end{matrix}
\end{matrix}
\end{equation}

%\noindent
%where $\sigma(i)$ is an indicator function. 




\subsection{Post-Processing}
\label{subsec:postprocessing}
Post-processing is an automatic post-editing process applied during decoding in the translation process.
The \textbf{\textit{Destandardizer}} uses the slot map dictionary generated by the Intent Parser to replace all keys in the standardized intent (i.e., \texttt{var0}, \texttt{var1}  and \texttt{var2}) with the corresponding memorized values (i.e., \texttt{dl}, \texttt{0xbb}, and \texttt{next\_cycle}). 

The generated snippet is then further post-processed using regular expressions (\textbf{\textit{Code Snippet Cleaning)}}. 
This operation includes the removal of (any) extra-spaces in the output (e.g., between operations and operands), and the removal of (any) extra-backslashes in escaped characters (e.g., \texttt{\textbackslash{\textbackslash{n}}}). Also, during the post-processing, the newline characters \texttt{\textbackslash{n}} are replaced with new lines to generate multi-line snippets.
As a final step, snippet tokens are joined to form a complete snippet (step \circled{6}).


\subsection{Implementation Details}
\label{subsec:implementation}

%\pietro{We performed a hyper-param fine-tuning. We can add this subsection in the experiment section.}
We implement the Seq2Seq model using {\fontfamily{qcr}\selectfont xnmt} \cite{neubig2018xnmt}. We use an Adam optimizer \cite{kingma2014adam} with $\beta_1=0.9$ and $\beta_2=0.999$, while the learning rate $\alpha$ is set to $0.001$. We set all the remaining hyper-parameters in a basic configuration: layer dimension = $512$, layers = $1$, epochs (with early stopping enforced) = $200$, beam size = $5$. %The last step is inference. 
% vocabulary size = $20,000$

Our CodeBERT implementation uses an encoder-decoder framework where the encoder is initialized to the pre-trained CodeBERT weights, and the decoder is a transformer decoder. The decoder is composed of $ 6$ stacked layers. The encoder follows the RoBERTa architecture~\cite{liu2019roberta}, with $12$ attention heads,  hidden layer dimension of $768$, $12$ encoder layers, $514$ for the size of position embeddings. We use the Adam optimizer~\cite{kingma2014adam}. The total number of parameters is 125M. The max length of the input is $256$ and the max length of inference is $128$. The learning rate $\alpha = 0.00005$, batch size = $32$, beam size = $10$, and train\_steps = $2800$.

==> tex/qualitative_old.tex <==
This section presents a qualitative evaluation using cherry- and lemon-picked examples from our test set. Several additional examples of success and failure cases are presented in the separate Appendix.

The first row in Table~\ref{tab:qualitative} demonstrates the ability of the approach to generate multi-line snippets from a relatively abstract intent. We note here that although the output would be considered incorrect based on automated metrics (e.g. BLEU-4), it is considered correct using the semantically and syntactically correct metrics. The output snippet produced by the approach is faithful to the natural language intent and compiles correctly under the NASM compiler. In the second row, we show another successful example of the generated output. 

The third and fourth show two examples of types of failure cases we observed in the output. The example in the third row illustrates an example of failure due to a lack of implicit knowledge. The natural language intent does not mention the indirect addressing mode (specified by the bracket [] in NASM syntax). In the fourth row, the example indicates a failure of the intent parser in recognizing explicitly stated identifiers in lengthier intents such as in the case of the \texttt{bh} register. 
The fifth row indicates another failure even while the intent seems simple, the standardization step fails in this case. We identify several paths for improvement through this qualitative evaluation, e.g. adding domain knowledge about assembly language to the Intent Parser. 




\begin{table*}[ht]
\caption{Illustrative examples of successful and failure cases. Errors are in red/bold.}
\label{tab:qualitative}
\begin{tabular}{ >{\centering\arraybackslash}m{3.5cm}|
 >{\centering\arraybackslash}m{3cm}|
 >{\centering\arraybackslash}m{3cm}}
\toprule
\textbf{Natural Language Intent}  & \textbf{Ground Truth Snippet}  & \textbf{Output} \\ \midrule
\textit{Put /bin/sh into ebx}  & \texttt{push 0x68732f2f} \textbackslash{}n \texttt{push 0x6e69622f} \textbackslash{}n \texttt{mov ebx, esp} & \texttt{push \textbf{long} 0x68732f2f} \textbackslash{}n \texttt{push \textbf{long} 0x6e69622f} \textbackslash{}n \texttt{mov ebx, esp}\\ \hline
\textit{Move esi into the doubleword} \textit{starting at the address esp-4} & \texttt{mov dword {[}esp-4{]}, esi}  & \texttt{mov dword {[}esp-4{]}, esi}  \\ \hline
\textit{Perform the xor operation between}  \textit{the location pointed by ecx and dh}  & \texttt{xor {[}ecx{]}, dh}  & \texttt{xor \textbf{\textcolor{red}{ecx, {[}dh{]}}}}   \\ \hline
\textit{Perform a logical xor between the address} \textit{specified by {[}ecx + 116{]} and bh register} \textit{and save the result in {[}ecx + 116{]}} & \texttt{xor {[}ecx + 116{]}, bh} & \texttt{xor byte {[}ecx + 116{]}, \textbf{\textcolor{red}{0x3}}}   \\ \hline
\textit{Declare the read label} & \texttt{read:} & \texttt{\textbf{\textcolor{red}{section:}}}   \\ \bottomrule
\end{tabular}
\end{table*}


